Timo: Towards Better Temporal Reasoning for Language Models

Reasoning about time is essential for Large Language Models (LLMs) to understand the world. Previous works focus on solving specific tasks, primarily on time-sensitive question answering. While these methods have proven effective, they cannot generalize to a wider spectrum of temporal reasoning tasks. Therefore, we propose a crucial question: Can we build a universal framework to handle a variety of temporal reasoning tasks? To that end, we systematically study 38 temporal reasoning tasks. Based on the observation that 19 tasks are directly related to mathematics, we first leverage the available mathematical dataset to set a solid foundation for temporal reasoning. However, the in-depth study indicates that focusing solely on mathematical enhancement falls short of addressing pure temporal reasoning tasks. To mitigate this limitation, we propose a simple but effective self-critic temporal optimization method to enhance the model's temporal reasoning capabilities without sacrificing general task abilities. Finally, we develop Timo, a model designed to excel in temporal reasoning at the 7B and 13B scales. Notably, Timo outperforms the counterpart LLMs by 10.0 and 7.6 in average accuracy scores and achieves the new state-of-the-art (SOTA) performance of comparable size. Extensive experiments further validate our framework's effectiveness and its generalization across diverse temporal tasks. The code is available at https://github.com/zhaochen0110/Timo.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table/all_subtasks_performance.tex <==
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{NiceTabular}{ccccccccc}[hvlines,cell-space-limits=8pt]
    \toprule
    \textsc{\textbf{Subtask}} & \textsc{\textbf{LLaMA2}} & \textsc{\textbf{TimeLLaMA}} & \textsc{\textbf{CodeLlama}} &
    \textsc{\textbf{WizardCoder}} & \textsc{\textbf{WizardMath}} &
    \textsc{\textbf{Tora}} & \textsc{\textbf{MAmmoTH}} & 
    \textsc{\textbf{Timo}}
    \\
    \midrule
    LLaMA2 & 55.0 & 52.1 & 54.0 & 69.5 & 85.0 \\
    \bottomrule
\end{NiceTabular}}
\caption{Results on 38 temporal tasks. For clarity, these tasks are grouped and displayed based on their associated time-related domains. The abbreviations \textsc{Amb., Arith., Dur., Freq., Caus., Rel., Typ.} refer to ambiguity resolution, arithmetic, duration, frequency, causality, relation and typical time, respectively. All values are percentages. Best results are in \textbf{bold}.}
\label{tab:main_table_all}
\end{table*}

==> table/analysis_combine.tex <==
\begin{table*}[t]
\centering
\begin{minipage}{0.45\linewidth}
\centering
\small
\begin{tabular}{l|cc}
\toprule
 & \textbf{Math-time} & \textbf{Pure-time} \\
\midrule
\textbf{\textsc{1 iter.}} &  \textbf{63.9} & \textbf{81.5} \\
\textbf{\textsc{2 iters}} &  62.1 & 80.9 \\
\textbf{\textsc{3 iters}} &  57.8 & 80.1 \\
\bottomrule
\end{tabular}
\caption{Performance comparison on different iteration settings.}
\label{tab:iteration}
\end{minipage}
\hfill
\begin{minipage}{0.50\linewidth}
\centering
\small
\begin{tabular}{l|cc}
\toprule
 & \textbf{Math-time} & \textbf{Pure-time} \\
\midrule
\textbf{\textsc{random}} &  61.5 & 79.8 \\
\textbf{\textsc{LLM-Judge}} & 61.3  & 80.2 \\
\textbf{\textsc{Timo}} &  \textbf{63.9} & \textbf{81.5} \\
\bottomrule
\end{tabular}
\caption{Performance comparison on different rewarding methods.}
\label{tab:prompt_comparison}
\end{minipage}
\end{table*}


==> table/analysis_inference.tex <==
% \begin{table}[ht]
\begin{wraptable}{r}{7cm}
\centering
\small
\begin{tabular}{l|ccc}
\toprule
  & \textbf{\textsc{Fs.}} & \textbf{\textsc{CoT}} & \textbf{\textsc{Math-CoT}} \\
\midrule
\textbf{\textsc{Amb.}} & 36.4 & 54.0 & \textbf{60.4} \\
\textbf{\textsc{Arith.}} & 23.6  & 46.3 & \textbf{52.1} \\
\textbf{\textsc{Dur.}} & 49.1  & 60.9 & \textbf{63.9 }\\
\textbf{\textsc{Freq.}} & 56.5  & 74.0 & \textbf{74.2 }\\
\midrule
\textbf{\textsc{Math tasks}}~$\dagger$ & 30.1  & 50.9 & \textbf{56.7} \\
\textbf{\textsc{Pure tasks}}~$\dagger$ & 61.1  & \textbf{69.3} & - \\
\bottomrule
\end{tabular}
\caption{Comparison between different prompting strategies under the inference period.}
\label{tab:study-inference}
\end{wraptable}
% \end{table}

==> table/case_cot.tex <==
\begin{table*}[t!]
\resizebox{\linewidth}{!}{
    \centering
\begin{tabular}{ll}
\toprule
\multicolumn{2}{c}{\bf{{TIMEX-NLI}}} \\ \hline
\textbf{Question}               & 
\begin{tabular}[c]{@{}l@{}}Answer the following question, select all the possible correct options, and each question has at least one correct option. \\
Premise: On Wednesday, they got married. \\
Hypothesis: Before Friday, they got married. \\
Options: A. Entailment B. Contradiction C. Neutral \\
\end{tabular}                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\textbf{TBench}                & 
\begin{tabular}[c]{@{}l@{}}
    Wednesday is before Friday. \\ As a result, we can infer that if something happens on Wednesday, it definitely happens before Friday. Therefore, the answer is A. Entailment.
\end{tabular} \\ \hline

\textbf{\textbf{TRAM}}      & 
\begin{tabular}[c]{@{}l@{}}
(1) \textit{Understanding
Context}: The premise is "On Wednesday, they got married." \\  
(2) \textit{Key Elements Extraction}: The key element is the marriage took place on Wednesday. \\ 
(3) \textit{Evaluation}:  The hypothesis states "Before Friday, they got married." \\
(4) \textit{Analysis and Comparison}: Since Wednesday is before Friday, the hypothesis aligns with the premise. \\
(5) \textit{Reasoned Conclusion}:The relationship between the premise and the hypothesis is Entailment. \\


  
\end{tabular}                                                                                \\ \toprule
\multicolumn{2}{c}{\bf{{Date Arithmetic}}} \\ \hline
\textbf{\textbf{Question}}      & 
What is the time 4 year and 1 month after Apr, 2000?                                                                  \\ \hline

\textbf{\textbf{TBench}}      & 
First, 4 years after 2000 is 2004. Next, 1 month after April is May. Therefore, 4 year and 1 month after Apr, 2000 is May, 2004.                                                               \\ \hline

\textbf{\textbf{TRAM}}     & 
\begin{tabular}[c]{@{}l@{}}
(1) \textit{Understanding
Context}: The task is to calculate the time that is 4 years and 1 month after April 2000. \\  
(2) \textit{Key Elements Extraction}: Start at April 2000; add 4 years; add 1 month. \\ 
(3) \textit{Evaluation}:  Adding 4 years to 2000 brings us to 2004. 
Adding 1 month to April brings us to May. \\
(4) \textit{Analysis and Comparison}: We need to ensure the calculations adhere to how we measure time, considering years and months. \\
(5) \textit{Reasoned Conclusion}: By combining the results of the evaluation, the time 4 years and 1 month after April 2000 is determined to be May 2004. \\


  
\end{tabular}                                                                                \\

\bottomrule
\end{tabular}}
    \caption{}
    % \vspace{-0.5em}
    \label{tb:cot}
\end{table*}



==> table/data_composition.tex <==
\begin{table*}[!t]
\centering
\small
\resizebox{\linewidth}{!}{%
\begin{tabular}{llllll}
\toprule
Training Dataset                                     & Type      & Annotation     & \# Samples        & Characteristics    & Fields    \\
\midrule
GSM8K                     & CoT       & Human          & 7K                & Grade Schol Exam   & $\coloredblock{Pre-Algebra}$  \\
{GSM8K-RFT}                  & CoT       & Llama          & 28K              & Llama + Validated &$\coloredblock{Pre-Algebra}$  \\
{AQuA-RAT}                   & CoT       & Human          & 90K               & GRE/GMAT Exam      &$\coloredblock{Inter-Algebra}$       \\
{MATH}                & CoT       & Human          & 7K                & Math Competition   & $\coloredblock{Pre-Algebra}$ $\coloredblock{Inter-Algebra}$ $\coloredblock{Algebra}$ $\coloredblock{Probability}$ 
$\coloredblock{NumTheory}$
$\coloredblock{Calculus}$ $\coloredblock{Geometry}$ \\
TheoremQA \FiveStarConvex  & CoT       & GPT-4          & 600              & GPT4 + Validated  &$\coloredblock{Algebra}$
$\coloredblock{Probability}$
$\coloredblock{NumTheory}$
$\coloredblock{Calculus}$
$\coloredblock{Geometry}$       \\
{Camel-Math }                     & CoT       & GPT-4          & 50K              & GPT4 (Unvalidated)  &$\coloredblock{Algebra}$
$\coloredblock{Probability}$
$\coloredblock{NumTheory}$
$\coloredblock{Calculus}$
$\coloredblock{Geometry}$    \\
College-Math \FiveStarConvex                         & CoT       & GPT-4          & 1.8K             & GPT4 (Unvalidated)  &$\coloredblock{Algebra}$    \\
\midrule
GSM8K \FiveStarConvex                                & PoT       & GPT4           & 14K              & GPT4 + Validated    &$\coloredblock{Pre-Algebra}$      \\ 
AQuA-RAT \FiveStarConvex                             & PoT       & GPT4           & 9.7K             & GPT4 + Validated     &$\coloredblock{Inter-Algebra}$      \\
MATH \FiveStarConvex                                 & PoT       & GPT4           & 7K               & GPT4 + Validated    &$\coloredblock{Pre-Algebra}$ $\coloredblock{Inter-Algebra}$ $\coloredblock{Algebra}$ $\coloredblock{Probability}$ \\
TheoremQA \FiveStarConvex                            & PoT       & GPT4           & 700              & GPT4 + Validated    &$\coloredblock{Algebra}$
$\coloredblock{Probability}$
$\coloredblock{NumTheory}$
$\coloredblock{Calculus}$
$\coloredblock{Geometry}$      \\
{MathQA}              & PoT       & Human          & 25K              & AQuA-RAT Subset   &$\coloredblock{Inter-Algebra}$      \\
{NumGLUE}                     & PoT       & Human          & 13K              & Lila Annotated  &  $\coloredblock{Pre-Algebra}$        \\
% {CrowdSourced \citep{mishra2022lila}}                & PoT       & Human          & 700              & Lila Annotated      
% & $\coloredblock{Algebra}$ $\coloredblock{Probability}$
% $\coloredblock{NumTheory}$
% $\coloredblock{Calculus}$ $\coloredblock{Geometry}$      \\
\midrule
\dataset& & &260K & &$\coloredblock{Pre-Algebra}$ $\coloredblock{Inter-Algebra}$ $\coloredblock{Algebra}$ $\coloredblock{Probability}$ 
$\coloredblock{NumTheory}$
$\coloredblock{Calculus}$ $\coloredblock{Geometry}$ \\
\bottomrule
\end{tabular}
}
\caption{Overview of our \dataset. \FiveStarConvex means with NEW rationales curated by us by prompting GPT-4. We have filtered out augmented samples that have answers inconsistent with the original dataset's annotations. Different colored squares represent different fields in mathematics: $\coloredblock{Pre-Algebra}$ Pre-Algebra; 
$\coloredblock{Inter-Algebra}$ Inter-Algebra;
$\coloredblock{Algebra}$ Algebra;
$\coloredblock{Probability}$ Probability;
$\coloredblock{NumTheory}$ NumTheory;
$\coloredblock{Calculus}$ Calculus;
$\coloredblock{Geometry}$ Geometry.}
\label{tab:flan}
\end{table*}

==> table/generalization.tex <==

\begin{table*}[ht]
\centering
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
 & \textbf{\textsc{GSM8K}} & \textbf{\textsc{MATH}} & \textbf{\textsc{NumGLUE}} & \textbf{\textsc{Per.}}\\
\midrule
\textbf{\textsc{SFT}} &  -33.61 & -17.46 & -10.31 &  +3.3 \\
\textbf{\textsc{TDPO}} &  \textbf{-7.71} & \textbf{-6.35} &  \textbf{-9.02} & \textbf{+7.5}\\
\bottomrule
\end{tabular}
\caption{Performance and forgetting rate  \\ comparison of SFT and our training methods}
\label{tab:generalization}
\end{table*}



==> table/mathinstruct.tex <==
\begin{table*}[]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{m{1.5cm}m{12cm}m{6cm}}
      \toprule
      \bf Type &\bf Instruction &\bf Output \\
      \hline
      \bf Multi-choice & How many ways can the letters in the word COMMON be arranged? Answer Choices: (A) 6 (B) 30 (C) 90 (D) 120 (E) 180 & Let's solve the multi-choice question step by step. According to the above .... \\ \hline
      \bf PoT & 	A team of six entered for a shooting competition. The best marks man scored 85 points. If he had scored 92 points, the average scores for. The team would have been 84. How many points altogether did the team score? Answer Choices: (A) 288 (B) 497 (C) 168 (D) 127 (E) 664. Let's program in Python in the response.& answers = ['A', 'B', 'C', 'D', 'E'] ...\\ \hline
      \bf CoT &  Tom paints a room that has 5 walls. Each wall is 2 meters by 3 meters. John can paint 1 square meter every 10 minutes. He has 10 hours to paint everything. How many hours does he have to spare? & Each wall is ... \\
      \bottomrule
    \end{tabular}}
    \caption{Templates}
    \label{tab:template}
\end{table*}
